Learning to Evade Static PE Machine Learning Malware Models via Reinforcement Learning

Machine learning is a popular approach to signatureless malware detection because it can generalize to never-before-seen malware families and polymorphic strains. This has resulted in its practical use for either primary detection engines or for supplementary heuristic detection by anti-malware vendors. Recent work in adversarial machine learning has shown that deep learning models are susceptible to gradient-based attacks, whereas non-differentiable models that report a score can be attacked by genetic algorithms that aim to systematically reduce the score. We propose a more general framework based on reinforcement learning (RL) for attacking static portable executable (PE) anti-malware engines. The general framework does not require a differentiable model nor does it require the engine to produce a score. Instead, an RL agent is equipped with a set of functionality-preserving operations that it may perform on the PE file. Through a series of games played against the anti-malware engine, it learns which sequences of operations are likely to result in evading the detector for any given malware sample. This enables completely black-box attacks against static PE anti-malware, and produces functional evasive malware samples as a direct result. We show in experiments that our method can attack a gradient-boosted machine learning model with evasion rates that are substantial and appear to be strongly dependent on the dataset. We demonstrate that attacks against this model appear to also evade components of publicly hosted antivirus engines. Adversarial training results are also presented: by retraining the model on evasive ransomware samples, a subsequent attack is 33% less effective. However, there are overfitting dangers when adversarial training, which we note. We release code to allow researchers to reproduce and improve this approach.

==> related_work.tex <==
There are several approaches to combating malware that utilize DGAs including blacklisting and DGA detection. In \cite{kuhrer2014paint} it was shown that public blacklists were surprisingly lacking in terms of DGA coverage with less than 1.2\% of DGAs analyzed by the authors being contained in any of the blacklists.  Private blacklists fared better, but had mixed results over families with coverage varying from 0\% to 99.5\%.  However, blacklists represent a reactionary countermeasure and cannot prevent novel attacks.  In order to prevent future attacks, malware researchers often must manually reverse engineer a malware sample to determine the DGA algorithm and pre-generate lists of DGA domains.  

DGA classifiers represent another strategy, often supplementary, to detect malware C\&C that relies on dynamically generated domain names.  DGA classifiers can potentially detect novel DGAs and in some cases, detect entirely new families of DGAs by generalizing from observed data. Classifying DGAs requires hand-crafted features (e.g., entropy, string length, vowel to consonant ratio, etc.) used to train a supervised learning model. This approach generally yields good results, however, there is an associated cost to the amount of manual work required to extract informative features. Additionally, new DGAs whose domains may be produced that are not well represented by the current feature set. Recrafting extracted features for each new DGA results in a resource-intensive adversarial game of cat and mouse. To mitigate this problem authors in \cite{antonakakis2012throw} presented a technique using Hidden Markov Models (HMMs) to detect DGAs.

Bulk predictions on large sets of domains were introduced by \cite{antonakakis2012throw, yadav2010detecting, yadav2012detecting}. Domain sets were clustered into groups to generate common statistical properties. Classification was performed using statistical tests (e.g., Kullback-Leibler divergence) to label clusters of potential DGAs. Researchers improved overall performance by including HTTP headers and other network-based contextual information, but those techniques highlight privacy and collection challenges  (i.e., not all networks can gather the same contextual information) \cite{aviv2011challenges}.

A summary of DGA detection algorithms and a novel approach based on long short-term memory networks (LSTM) which operates on only the domain name (no contextual information) can be found in \cite{woodbridge2016DGA}, which boasts F1 scores exceeding 99\% for detecting never-before-seen domains from common DGA families. This technique relies solely on the domain string and requires no additional features or contextual information. The authors stress the LSTM approach is not to replace any one technique, but rather be implemented symbiotically as suggested in \cite{antonakakis2012throw} to further improve the efficacy of detecting DGAs.
